Learned Video Codec with Enriched Reconstruction for CLIC P-frame Coding

This paper proposes a learning-based video codec, specifically used for Challenge on Learned Image Compression (CLIC, CVPRWorkshop) 2020 P-frame coding. More specifically, we designed a compressor network with Refine-Net for coding residual signals and motion vectors. Also, for motion estimation, we introduced a hierarchical, attention-based ME-Net. To verify our design, we conducted an extensive ablation study on our modules and different input formats. Our video codec demonstrates its performance by using the perfect reference frame at the decoder side specified by the CLIC P-frame Challenge. The experimental result shows that our proposed codec is very competitive with the Challenge top performers in terms of quality metrics.

==> images/ablation-larb.tex <==
\begin{figure*}
\centering
{
\begin{tabular}{cc}
\(r_t\) & \(\hat{r}_t\) \\
\includegraphics[width=0.45 \textwidth]{images/examples/2/r_frame.png}&
\includegraphics[width=0.45 \textwidth]{images/examples/2/r_hat.png}\\
(a) & (b)\\
\end{tabular}

\begin{tabular}{cc}
\(x_{t-1}\) & \(x_t\)\\
\includegraphics[width=0.45 \textwidth]{images/examples/2/x_frame.png} & 
\includegraphics[width=0.45 \textwidth]{images/examples/2/y_frame.png}\\

(c) & (d)\\
\end{tabular}

\begin{tabular}{cc}
\(x_{t-1} + \hat{r}_t\) & \(\hat{x}_t\) \\
\includegraphics[width=0.45 \textwidth]{images/examples/2/y_before_hat.png}&
\includegraphics[width=0.45 \textwidth]{images/examples/2/y_hat.png}\\

(e) & (f)\\
\end{tabular}

\caption{Comparison for OpenDVC ME-Net and Our ME-Net.}

\label{fig:example-refine-net-motion-img}
}
%\vspace{-0.1cm}


\vspace{-0.3cm}
\end{figure*}

==> images/ablation.tex <==
\begin{figure}[hb!]
  \centering
  \centering
  {
      \begin{tabular}{cc}
      \includegraphics[width=0.5\columnwidth]{images/png/abl-curve-msssim.png}&
      \includegraphics[width=0.5\columnwidth]{images/png/abl-refine-msssim.png}\\
      \end{tabular}
      \caption{(a) Our Y+U+V model outperforms RGB and YUV channel in all bits-per-pixel. (b) The compressor model comparison for residual information and motion vector. }
  \label{fig:rgb-vs-yuv-compressor}
  }
\end{figure}

==> images/clic-result.tex <==
\begin{figure}[hb!]
  \centering
      {
        \begin{tabular}{cc}
        \includegraphics[width=0.465 \columnwidth]{images/png/rd-curve-psnr.png}&
        \includegraphics[width=0.485 \columnwidth]{images/png/rd-curve-msssim.png}\\
        \end{tabular}
        \caption{The evaluation on CLIC test set. Our scheme competes with the top performer in the leader board.}
      \label{experiment-result}
    }
    \hspace{-0.1cm}
\end{figure}

==> images/larb.tex <==
\begin{figure}[hb!]
  \centering

  {
  \includegraphics[width=0.93\columnwidth]{images/png/larb.png}
  }
  \caption{Our Local Attention Residual Block (LARB) exploits multi-scale information from the input feature. We employ bilinear upsampling in the upscaling process.}
  \label{fig:larb-img}
  \vspace{-0.3cm}
\end{figure}

==> images/me-training.tex <==
\begin{figure*}
\centering
{
\begin{tabular}{c}
\includegraphics[width=0.95 \textwidth]{images/png/me-training.png}\\
\end{tabular}

\caption{Our ME-Net Training: The motion estimation is performed using downsampled frame and enhanced further. We use MSE in each stage to optimize the Motion Enhancement. }

\label{fig:me-net-training-img}
}
%\vspace{-0.1cm}


\vspace{-0.3cm}
\end{figure*}

==> images/synthesis-net-residual.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{images/pdf/synthesis-net-residual.pdf}
  \caption{The synthesis effect in residual coding. With end-to-end training, the synthesis-net using signals from residual decoder to reconstruct current frame. The synthesis output can be targeted for specific distortion loss at the time of training. As shown in \(\hat{x}_t\), the model is targeted for MS-SSIM.}
  \label{fig:synthesis-net-residual-img}
\end{figure*}
